Minimizing Total Busy Time for Energy-Aware Virtual Machine Allocation Problems

This paper investigates the energy-aware virtual machine (VM) allocation problems in clouds along characteristics: multiple resources, fixed interval time and non-preemption of virtual machines. Many previous works have been proposed to use a minimum number of physical machines, however, this is not necessarily a good solution to minimize total energy consumption in the VM placement with multiple resources, fixed interval time and non-preemption. We observed that minimizing the sum of total busy time of all physical machines implies minimizing total energy consumption of physical machines. In addition to, if mapping of a VM onto physical machines have the same total busy time then the best mapping has physical machine's remaining available resource minimizing. Based on these observations, we proposed heuristic-based EM algorithm to solve the energy-aware VM allocation with fixed starting time and duration time. In addition, this work studies some heuristics for sorting the list of virtual machines (e.g., sorting by the earliest starting time, or latest finishing time, or the longest duration time first, etc.) to allocate VM. We evaluate the EM using CloudSim toolkit and jobs log-traces in the Feitelson's Parallel Workloads Archive. Simulation's results show that all of EM-ST, EM-LFT and EM-LDTF algorithms could reduce total energy consumption compared to state-of-the-art of power-aware VM allocation algorithms. (e.g. Power-Aware Best-Fit Decreasing (PABFD) [7])).

==> acmcccode.tex <==
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003033.10003099.10003100</concept_id>
<concept_desc>Networks~Cloud computing</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003752.10003809.10010047.10010048.10003808</concept_id>
<concept_desc>Theory of computation~Scheduling algorithms</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10010940.10010941.10010942.10010948</concept_id>
<concept_desc>Software and its engineering~Virtual machines</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10010520.10010521.10010537</concept_id>
<concept_desc>Computer systems organization~Distributed architectures</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Networks~Cloud computing}
\ccsdesc[500]{Theory of computation~Scheduling algorithms}
\ccsdesc[300]{Software and its engineering~Virtual machines}
\ccsdesc[300]{Computer systems organization~Distributed architectures}


%
% End generated code
%

\printccsdesc


\keywords{Cloud Computing; Resource Management; Green IT; Energy efficiency; Virtual machine allocation; EVMAP}

==> fig-algo.tex <==
\begin{algorithm*}[!hbt]
\caption{EMinRET-ST and EMinRET-FT: Heuristics for energy-aware VM allocation in HPC Clouds}\label{alg:remindft}
\begin{algorithmic}[1]

\Function{EMinRET-ST}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByStartTime( vmList ) \Comment{1}\label{line:sortbystarttime}
\State return EMinRET( vmList, hostList )
\EndFunction

\Function{EMinRET-FT}{}
\State	\textit{Input:} vmList - a list of virtual machines to be scheduled
\State	\textit{Input:} hostList - a list of physical servers
\State	\textit{Output:} mapping (a feasible schedule) or null % \khanh{should be ``null''?. OK}
\State	vmList = sortVmListByFinishTime( vmList ) \Comment{2}\label{line:sortbyfinishtime}
\State return EMinRET( vmList, hostList )
\EndFunction

\end{algorithmic}
\end{algorithm*}



==> referenc.tex <==
\begin{thebibliography}{4}

%\bibitem{Albers2010} Albers, S. and Fujiwara, H.: Energy-efficient algorithms, ACM Review, Vol. 53, No. 5, pp. 86-96. (2010), doi: 10.1145/1735223.1735245
\bibitem{Albers2010} Albers, S.: Energy-efficient algorithms. Commun. ACM 53(5), 86–96 (2010)

\bibitem{Ittner2007} Barroso, L.A., H\"{o}lzle, U.: The Case for Energy-Proportional Computing. Computer 40(12), 33–37 (2007)

\bibitem{Beloglazov2012} Beloglazov, A., Abawajy, J., Buyya, R.: Energy-aware Resource Allocation Heuristics for Efficient Management of Data Centers for Cloud Computing. Future Generation Computer Systems 28(5), 755–768 (2012)

\bibitem{Beloglazov2011} Beloglazov, A. and Buyya, R.: Optimal Online Deterministic Algorithms and Adaptive Heuristics for Energy and Performance Efficient Dynamic Consolidation of Virtual Machines in Cloud Data Centers, CONCURRENCY AND COMPUTATION: PRACTICE AND EXPERIENCE, Concurrency Computat.: Pract. Exper., pp. 1-24, (2011), doi: 10.1002/cpe

\bibitem{Buyya2009a} Buyya, R., Yeo, C., Venugopal, S., Broberg, J., Brandic, I.: Cloud computing and emerging IT platforms: Vision, hype, and reality for delivering computing as the 5th utility. Future Generation Computer Systems 25(6), 599–616 (2009)

\bibitem{Fan2007a} Fan, X., Weber, W.-D., Barroso, L.A.: Power provisioning for a warehouse-sized computer. ACM SIGARCH Comput. Archit. News. 35, 13 (2007)

%\bibitem{Goiri2010} Goiri, \'{I}., Nou, R., Berral, J., Guitart, J., Torres, J.: Energy-aware Scheduling in Virtualized Datacenters. In: IEEE International Conference on Cluster Computing, CLUSTER 2010, pp. 58–67 (2010)

\bibitem{Hung2011} Quang-Hung, N., Thoai, N., Son, N.T.: Performance constraint and power-aware allocation for user requests in virtual computing lab, Journal of Science and Technology (Vietnam), vol. \textbf{49}, No. 4A, pp. 383-392 (2011.)

%\bibitem{GAPA} Quang-Hung, N., Nien, P. D., Nam, N. H., Tuong, N. H., and Thoai, N..: A Genetic Algorithm for Power-Aware Virtual Machine Allocation in Private Cloud, ICT-EurAsia’13, vol. LNCS \textbf{7804}, pp. 183--191. (2013) doi: 10.1007/978-3-642-36818-9\_19

\bibitem{Hung2013}Quang-Hung, N. et al.: EPOBF: Energy Efficient Allocation of Virtual Machines in High Performance Computing Cloud. J. Sci. Technol. Vietnamese Acad. Sci. Technol. 51, No. 4B, Special on International Conference on Advanced Computing and Applications (ACOMP2013), 173–182 (2013).

\bibitem{HungGPUGA2014} Quang-Hung, N. et al.: A GPU-Based Enhanced Genetic Algorithm for Power-Aware Task Scheduling Problem in HPC Cloud. ICT-EurAsia 2014. LNCS 8407, 159–169 (2014).

\bibitem{Le2011} Le, K. et al.: Reducing electricity cost through virtual machine placement in high performance computing clouds. In: Lathrop, S. et al. (eds.) Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis on - SC ’11. p. 1 ACM Press, New York, USA (2011).

\bibitem{Mauch2013} Mauch, V. et al.: High performance cloud computing. Futur. Gener. Comput. Syst. 29, 6, 1408–1416 (2013).

\bibitem{Sotomayor2008} Sotomayor, B., Keahey, K., Foster, I.: Combining batch execution and leasing using virtual machines. In: Proceedings of the Eighteenth International Symposium on High Performance Distributed Computing (HPDC’08), Boston, MA, USA, 23–27 June 2008, pp. 87–96 (2008)

%\bibitem{Sotomayor2009c} Sotomayor, B. and Ignacio, M. and Foster, I.: Resource Leasing and the Art of Suspending Virtual Machines, The 11th IEEE International Conference on High Performance Computing and Communications (HPCC-09),  pp. 59-68. IEEE Computer Society Washington, DC, USA (2009) doi: 10.1109/HPCC.2009.17

\bibitem{Sotomayor2010} Sotomayor, B.: Provisioning Computational Resources Using Virtual Machines and Leases,  PhD Thesis submited to The University of Chicago, US, (2010)

\bibitem{Speitkamp2010} Speitkamp, B., Bichler, M.: A mathematical programming approach for server consolidation problems in virtualized data centers. Serv. Comput. 3, 266–278 (2010)

\bibitem{VonLaszewski2009} von Laszewski, G., Wang, L., Younge, A.J., He, X.: Power-aware scheduling of virtual machines in DVFS-enabled clusters. In: IEEE Intl. Conf. on Cluster Computing and Workshops, 2009, pp. 1–10 (2009), doi:10.1109/CLUSTR.2009.5289182

\bibitem{Panigrahy2011} Panigrahy, R., Talwar, K., Uyeda, L., Wieder, U.: Heuristics for vector bin packing. Technical report, Microsoft Research (2011)

\bibitem{Pham2010} Pham, T.V. et al.: A service composition framework for market-oriented high performance computing cloud. Proceedings of the 19th ACM International Symposium  on High Performance Distributed Computing - HPDC ’10. p. 284 ACM Press, New York, New York, USA (2010).

\bibitem{Feitelson2004} Feitelson, D.G., Rudolph, L., Schwiegelshohn, U.: Parallel job scheduling - a status report. In: Feitelson, D.G., Rudolph, L., Schwiegelshohn, U. (eds.) JSSPP 2004. LNCS, vol. 3277, pp. 1–16. Springer, Heidelberg (2005)

\bibitem{Garg2009} Garg, S.K., Yeo, C.S., Anandasivam, A., Buyya, R.: Energy-Efficient Scheduling of HPC Applications in Cloud Computing Environments. arXiv Prepr. arXiv0909.1146 (2009)

\bibitem{Vis2011} Viswanathan, H. et al.: Energy-Aware Application-Centric VM Allocation for HPC Workloads. 2011 IEEE International Symposium on Parallel and Distributed Processing Workshops and Phd Forum. pp. 890–897 IEEE (2011).

\bibitem{Cloudsim} Calheiros, R.N. et al.: CloudSim: a toolkit for modeling and simulation of cloud computing environments and evaluation of resource provisioning algorithms. Softw. Pract. Exp. 41, 1, 23–50 (2011).

\bibitem{Tako2012} Takouna, I. et al.: Energy efficient scheduling of HPC-jobs on virtualize clusters using host and VM dynamic configuration. ACM SIGOPS Oper. Syst. Rev. 46, 2, 19 (2012).

\bibitem{Maam2011} M\"{a}mmel\"{a}, O. et al.: Energy-aware job scheduler for high-performance computing. Comput. Sci. - Res. Dev. 27, 4, 265–275 (2011).

%\bibitem[Spec1]{Spec1} SPECpower ssj2008 results for Fujitsu Siemens Computers PRIMERGY RX200 S4 (Intel Xeon L5430). \url{http://bit.ly/LvmII4}

%\bibitem{Spec2} SPECpower ssj2008 results for HP ProLiant DL585 G5 (2.70GHz, AMD Opteron 8384). \url{http://bit.ly/JrkskF}

%\bibitem{Spec3} SPECpower ssj2008 results for HP ProLiant DL785 G5 (2.30GHz, AMD Opteron 8376 HE). \url{http://bit.ly/K99RfD}

%\bibitem{SDSC} The San Diego Supercomputer Center (SDSC) Blue Horizon log. \url{http://bit.ly/JUQsiP}
\bibitem{WorkloadLPC} The LPC log from the Parallel Workloads Archive. \url{http://www.cs.huji.ac.il/labs/parallel/workload/l\_lpc/LPC-EGEE-2004-1.2-cln.swf.gz}. Last accessed: 30-January-2014

\bibitem{AmazonEC2HPC}  http://aws.amazon.com/hpc/

\end{thebibliography}


==> theorems.tex <==
\subsection{Theorems}
\label{sec:theorems}

%% \textit{Theorem 1:}

\begin{thm}
\label{sec:theorem01}
Given a cloud system with a set of identical physical machines, 
assume that power consumption of a physical machine is $P(u) = b + au$, 
in which: 
 $b = P_{idle}$ is the idle power consumption, 
 $a = P_{max} - P_{idle}$ is the maximum power consumption, and
 $u$ is the CPU utilization in percentage ($0 \leq u \leq 1$).
 We denote $e_{ij}$ is energy consumption of each virtual machine $i$-th that is scheduled on any physical machine $j$-th.
 If the $u$ of the mapped virtual machine is a constant, 
 then the energy consumption of each virtual machine, $e_{ij}$, is independent of any mapping (i.e. any schedule). 
 We have $\forall i \in {1,2,...,n}, j \in {1,2,...,m}: e_{ij} = e_{i}$.
\end{thm}

 %% \textit{Proof:} 
\begin{proof}
Recall that the energy consumption is formulated in Equation (\ref{eq:energy}), 
 and power consumption, $P(u)$, is a linear function of CPU utilization, $u$. 
 Therefore for all $ i \in {1,2,...,n}$ and $j \in {1,2,...,m}$, we see that $e_{ij}$ is the integral of the $P(u)$ over any time interval [$t_{1}$, $t_{2}$],
and is the same value, denoted as $e_{i}$.
%% $\square$
\end{proof}

From Theorem \ref{sec:theorem01}, we can imply the following theorem.

%% \textit{Theorem 2:}
\begin{thm}
\label{sec:theorem02}
 If all physical machines are homogeneous then minimizing total energy consumption is equivalent to
 minimizing the sum of total completion time of all physical machines ($\sum_{j=1}^{m} T_{j}$).
 
\begin{equation}
\label{eq:minimize2}
\textbf{Minimize} \   ( E_j^{0} \times \sum_{j=1}^{m} T_{j}  +  \sum_{i=1}^{n} e_{i} ) ~ \sim ~ \textbf{Minimize} \   ( \sum_{j=1}^{m} T_{j})
\end{equation}  

\end{thm}

%% \textit{Proof:} 
\begin{proof}
According to the objective function
described in (\ref{eq:minimize}), we have all physical machines are identical machine, i.e. $\forall j=1,2,..., m : E_j^0 $ is constant and
$e_i$ is independent of any mapping (i.e. any schedule). 
%% $\square$
\end{proof}

Based on the above observations, we propose our energy-aware algorithms denoted as EMinRET
which is presented in the next section.
 %% \ref{sec:schedalgo}.
%We assume that all physical machine are homogeneous.

